A Simple Algorithm for Consistent Query Answering under Primary Keys

We consider the dichotomy conjecture for consistent query answering under primary key constraints. It states that, for every fixed Boolean conjunctive query q, testing whether q is certain (i.e. whether it evaluates to true over all repairs of a given inconsistent database) is either polynomial time or coNP-complete. This conjecture has been verified for self-join-free and path queries. We propose a simple inflationary fixpoint algorithm for consistent query answering which, for a given database, naively computes a set $\Delta$ of subsets of facts of the database of size at most k, where k is the size of the query q. The algorithm runs in polynomial time and can be formally defined as: (1) Initialize $\Delta$ with all sets $S$ of at most $k$ facts such that $S\models q$. (2) Add any set $S$ of at most k facts to $\Delta$ if there exists a block $B$ (i.e., a maximal set of facts sharing the same key) such that for every fact $a \in B$ there is a set $S' \subseteq S \cup \{a\}$ such that $S'\in \Delta$. For an input database $D$, the algorithm answers "q is certain" iff $\Delta$ eventually contains the empty set. The algorithm correctly computes certainty when the query q falls in the polynomial time cases of the known dichotomies for self-join-free queries and path queries. For arbitrary Boolean conjunctive queries, the algorithm is an under-approximation: the query is guaranteed to be certain if the algorithm claims so. However, there are polynomial time certain queries (with self-joins) which are not identified as such by the algorithm.

==> X+LowerBound.tex <==
%!TeX root = main.tex


% \newcommand{\allB}{\mathbb{B}}
% \newcommand{\allE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}

% \newcommand{\back}{U}
% \newcommand{\front}{V}

The proof that $\Cqk$ fails to capture $\certain(q)$ is done in three steps.
The first step shows, via a combinatorial argument, that the "self-join" query
\AP
\[
  \intro*\qFour \defeq R(\underline{x}\, yz) \land R (\underline{z}\, xy)
\] 
is such
that $\certain(\qFour)$ cannot be computed using $\Cqk(\qFour)$, for no choice
of $k$.
%
In a second step, we show that the
"self-join-free query" 
\AP
\[
  \intro*\qFive \defeq R_1(\underline{x}\, y) \land S_1(\underline{y z}\, x)
\]
satisfies the same property: $\certain(\qFive)$ 
cannot be computed using $\Cqk(\qFive)$ for any choice of $k$. This is shown
by reducing the case of $\qFive$ to the case of $\qFour$. Finally, we prove the
same property for \emph{any} "self-join-free query" $q$ such that $q\not\models\HP$
by reducing the case of $\qFive$ to such query $q$.

\subsubsection{The case of $\qFour$}

Note that the query $\qFour$ is not a "self-join-free query". In particular, we
can have $D \models \qFour(aa)$ for some fact $a\in D$. We call ""self-loops"" such solutions.

% A database $D$ contains a self-loop if there exists a self-loop
% solution to $\qFour$. The next observation proves that we can safely ignore
% such self-loops.

% \begin{prop}
% \label{prop-no-self-loop-q4}
% Let $D$ be a database instance of $\qFour$ that contains self-loops. Then one of the following holds:
% \begin{enumerate}
% \item There exists a "block" $B$ in $D$ such that for every "fact" $a\in B$ we have $D\models q(aa)$
% \item There exists a database $D'$ that does not contain self-loop such that $D\models \certain(\qFour)$ iff $D'\models \certain(\qFour)$. Moreover we can obtain such a $D'$ from $D$ very efficiently (via \fo translation). 
% \end{enumerate} 
% \end{prop}
% \begin{proof}
% Assume that $(1)$ is false. Then every "block" $B$ in $D$ has some $a\in B$ such that $D\not\models q(aa)$. Define $D'$ be simply deleting all facts $a$ that are involved in self-loops. By assumption, every "block" $B$ in $D$  corresponds to a block $B'$ in $D'$ such that $B'\subseteq B$ and $B'\ne \emptyset$. 

% Now we verify $(2)$. Suppose $D'\not\models \certain(\qFour)$ then there is a repair $r'$ of $D'$ such that $r'\not\models \qFour$. But $r'$ is also a repair of $D$ and hence $D\not\models \certain(\qFour)$. Conversely if $D\not\models \certain(\qFour)$ then there is a repair $r$ of $D$ such that $r\not\models \qFour$. But then for any fact $a$, if $a$ is involved in a self-loop then $a\not\in r$. This implies that every $a\in r$ is also present in $D'$. Hence $r$ is also a repair of $D'$ and hence $D'\not\models \certain(\qFour)$.

% \end{proof}

% Note that the construction of $D'$ from $D$ is trivial and the first condition can be expressed in \fo. So wihtout loss of generality we will assume that the input database instances do not contain self-loops.
To prove that $\Cqk(\qFour)$ does not compute $\certain(\qFour)$ for any choice
of $k$, we actually prove a stronger statement: not even an extension
``$\Cqkp(\qFour)$'' of $\Cqk(\qFour)$ can capture $\certain(\qFour)$. This
stronger form will be needed later for reducing $\qFive$ to $\qFour$.

Let us first explain the extension which is tailored to two-atom queries (thus,
strictly speaking, it `extends' $\Cqk(\qFour)$ only in this context). Recall
that the definition of $\Cqk(q)$ iteratively adds a "$k$-set" $S$ to
$\Deltak(q,D)$ if there exists a "block" $B$ of $D$ such that for every "fact"
$u\in B$ there exists $S' \subseteq S\cup \{ u\}$ such that
$S' \in \Deltak(q,D)$.  \AP This rule guarantees the invariant property
\eqref{eq:Delta:invariant}: for all $S \in \Deltak(q,D)$ and all "repair" $r$
of $D$ containing $S$, we have $r\models q$.

\AP The algorithm $\intro*\Cqkp(q)$ initializes the set $\intro*\Deltakp(q,D)$
of "$k$-sets" as in $\Cqk(q)$, and inherits the aforementioned derivation rule
of $\Cqk(q)$, but it contains also a second derivation rule: A "$k$-set" $S$ is
also added to $\Deltakp(q,D)$ if there exists a "fact" $a$ of $D$ such that a
is not a self-loop and for
every "fact" $u \in \set{ b \in D : D \models q(ab) \lor q(ba) \lor a=b }$
there exists $S' \subseteq S\cup \set{u}$ such that $S' \in \Deltakp(q,D)$. As before, we define $\Cqkp(q)$ to accept if the empty set is eventually derived.

Let us verify that the invariant property \eqref{eq:Delta:invariant} remains true:
\begin{align}
  \textit{For every "repair" $r$ of $D$ and every $S\in \Deltakp(q,D)$, if $S\subseteq r$ then $r\models q$.}  \tag{$\textsc{Inv}^+$}\label{eq:Delta:invariantplus}
\end{align}
To see this,
consider a "repair" $r$ containing a "$k$-set" $S$ of "facts" from $\Deltakp(q,D)$, and let us show \eqref{eq:Delta:invariantplus}
by induction on the number $n$ of steps in which $S$ was derived. The case $n=0$ is trivial, and so is the induction step where $S$ was derived using the first derivation rule. So, suppose $S$ was derived using the second derivation rule, by the existence of a "fact" $a$ from $D$.
If $r$ contains any $u \in \set{ b \in D : D \models q(ab) \lor q(ba) \lor a=b }$
then a subset of $S \cup \set u$ was derived in less than $n$ steps, and hence by induction hypothesis $r\models q$. 
Otherwise, let $r'$ be the "repair" constructed
from $r$ by selecting $a$ for the "block" of $a$. By the previous argument, $r'\models q$. 
By hypothesis there is no "fact" $b$ in $r$ such that $q(ab) \lor q(ba)$  and
since the fact a is not a self-loop, we have $r' \setminus \set a \models q$,
which implies $r\models q$. 


Note that as is the case for $\Cqk(q)$, $\Cqkp(q)$ also runs in polynomial time and may only give a ``false negative'' over self-loop free database instances.
We can now formally state the first contribution of this section:
\begin{thm}
\label{thm-X+lowerBound}
  \AP
 $\certain(\qFour)$ cannot be computed by
  $\Cqkp(\qFour)$, for any choice of $k$.
\end{thm}

Before proving \Cref{thm-X+lowerBound} we discuss some special properties of the query
$\qFour$. Note that $\qFour$ is a "self-join" two-atom query. 
\AP
We define the ""solution graph"" of $D$, denoted by $\intro*\solgraph$, to be an undirected graph whose vertices are the "facts" of $D$ and it contains an edge $\set{a,b}$ whenever $D \models \qFour(ab)$ holds. In the context of "solution graphs", a ""triangle"" is just a clique on three vertices (without self-loops).

We first state some key properties of $\qFour$ for any "database" $D$ and "facts" $a,b,c\in D$:
\begin{enumerate}
  \item if $D \models \qFour(ab) \land \qFour(ac)$ then $b= c$,
  \item if $D \models \qFour(ba) \land \qFour(ca)$ then $b= c$,
  \item if $D\models \qFour(ab) \land \qFour(bc)$ then $D\models \qFour(ca)$,
  \itemAP hence, every connected component of $\solgraph$ is either a "triangle", a 2-clique (without self-loops), or a single vertex (with or without a self-loop).\label{shape-solgraph-q4}
\end{enumerate}


\knowledgenewrobustcmd{\Dn}[1][n]{\cmdkl{D_{#1}}}
We now prove that for all $k$, $\Cqkp(\qFour)$ does not compute
$\certain(\qFour)$. To this end, for every $n \geq 4$ we exhibit a "database"
$\Dn$ such that
\begin{itemize}
  \item $\Dn \models \certain(\qFour)$ (\Cref{prop-Dk in certain}), and
  \item $\Dn[n] \not\models \Cqkp[n-2](\qFour)$ (\Cref{prop-Dk not in Delta(k-2)}).
\end{itemize}
Intuitively, the "database" $\Dn$ has $n$ "blocks" of the form
$B_1,\cdots,B_n$ where each $B_i$ consists of $n-1$ "facts" denoted
$b_i^1,\cdots,b_i^{n-1}$. Further, $\Dn$ also has $(n-1)(n-3)$ "blocks" of the
form $E^j_l$ for every $1\leq j \leq n-1$ and $1\leq l \leq n-3$, where each
$E_l^j$ has two "facts" denoted by $u_l^j$ and $v_l^j$.  The "solution graph" of
$\Dn$ is depicted in \Cref{fig:counterexample}.

  \begin{figure}
    \centering
    \includegraphics[width=\textwidth]{img/counterexample.pdf}
    \caption{"Solution graph" for "database" $\Dn$. Black dots denote "facts",
      rectangles denote "blocks", and three-pointed edges denote "triangles" ("ie", 3-cliques) in the
      "solution graph" of $\Dn$.  There are $n-1$ "facts" in each "block" $B_i$ and two "facts" in each "block" $E^j_k$.}
    \label{fig:counterexample}
  \end{figure}

\AP
\paragraph{Definition of $\intro*\Dn$}
We now formally define the "facts" of the "database" $\Dn$. Fix some $n\ge 4$.
Define $n$ "blocks" of the form
$B_1,\cdots,B_n$ in $\Dn$
where each $B_i$ consists of $n-1$ "facts" denoted
$b_i^1,\cdots,b_i^{n-1}$ and $(n-1)(n-3)$ "blocks" of the form
$E^j_l$ for $1\leq j \leq n-1, 1\leq l \leq n-3$, where each $E_l^j$ have two "facts" denoted by
$u_l^j$ and $v_l^j$. 


Let $a_1,\cdots,a_n$ and  $e_i^j$ where $1\leq j \leq n-1, 1\leq i \leq n-3$ be fresh active domain elements.
The "facts" of $\Dn$ are defined as follows.
%
\begin{itemize}
\item $b_1^j=(\underline{a_1}~~ a_2e^j_1)$,
  $b_2^j = (\underline{a_2}~~e^j_1a_1)$;
\item for every $3 \le i \le n-2$:~~~
  $b^j_i = (\underline{a_i}~~e^j_{i-2}e^j_{i-1})$;
\item $b^j_{n-1} = (\underline{a_{n-1}}~~ e^j_{n-3}a_{n})$ and
$b^j_{n} = (\underline{a_{n}} ~~ a_{n-1}e^j_{n-3})$;
%\item for every $1\le j \le n-1$ we have:
%\begin{itemize}
\item $u_1^j=(\underline{e^j_1}~~a_1a_2)$ and
  $v_{n-3}^j=(\underline{e^j_{n-3}}~~a_{n}a_{n-1})$;
\item for every $1\le l < n-3$:~~ $v_l^j=(\underline{e^j_l}~~e^j_{l+1}a_{l+2})$
  and $u_{l+1}^j=(\underline{e^j_{l+1}}~~a_{l+2}e^j_{l})$.
%\end{itemize}
\end{itemize}

As shown in \Cref{fig:counterexample:triangles}, it can be verified that for every $1\le j \le n-1$ we have the "triangles" $\{b^j_1,b^j_2,u^j_1\}$ and
$\{b^j_{n-1},b^j_{n}, v^j_{n-3}\}$ and for every $1\le l < n-3$ we have a "triangle"
$\{v^j_l,u^j_{l+1},b^j_{l+2}\}$. We get the "solution graph" described in Figure~\ref{fig:counterexample}.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{img/counterexample-triangles.pdf}
  \caption{"Triangles" in the "database" $\Dn$.}
  \label{fig:counterexample:triangles}
\end{figure}

\bigskip



$\Dn$ is defined in such a way that every "fact" of $\Dn$ is part of a
"triangle".  More precisely, we have the following "triangles" in the "solution
graph" of $\Dn$: For every $1\le j \le n-1$, the triples $\{b^j_1,b^j_2,u^j_1\}$
and $\{b^j_{n-1},b^j_{n}, v^j_{n-3}\}$ form "triangles" and for every
$1\le l < n-3$ we have a "triangle" $\{v^j_l,u^j_{l+1},b^j_{l+2}\}$. 

\begin{prop}
\label{prop-Dk in certain}
For every $n\ge 4$, $\Dn \models \certain(\qFour)$.
\end{prop}
\begin{proof}
Fix some $n\ge 4$ and consider the "database" $\Dn$. Let $B_1,\ldots B_n$ be the "blocks" of $\Dn$. Now for every $1\le j \le n-1$ if a "repair" $r$
  contains two $i,i'$ such that $b^j_i, b^j_{i'}\in r$ then it is easy to
  verify that $r\models q$ (\cf~Figure~\ref{fig:counterexample}).
  
  Now since each $B_i$ contains exactly $n-1$ "facts" of the form
  $b^1_i,\ldots ,b^{n-1}_i$, by the pigeonhole principle, every "repair" $r$ must
  contain two $i,i'$ such that $b^j_i, b^j_{i'}\in r$. Hence, every "repair" $r$ verifies $r\models q$.
\end{proof}


It remains to prove the following:
\begin{prop}
\label{prop-Dk not in Delta(k-2)}
Let $k\geq 2$. $\Dn[k+2] \not\models \Cqkp(\qFour)$.
\end{prop}

%\begin{proofsketch}
%  To prove the proposition, for a set of "blocks" $\XX =\{X_1, \dots X_k\}$ of
%  $\Dn[k+2]$, if $W = \{a_1,\ldots a_k\}$ is a set of facts where each
%  $a_i\in X_i$, then we call $W$ a "partial repair" of $\XX$. Further, $W$ is
%  called an \defstyle{obstruction set} of $\XX$ if $W$ satisfies some
%  ``desired properties''. In particular we will show that if $W$ is an
%  obstruction set then $W\not\models \qFour$. Next we will prove that for any
%  set of "blocks" $\XX =\{X_1, \dots X_k\}$ of $\Dn[k+2]$, we can always pick a
%  "partial repair" $W$ of $\XX$ such that $W$ is an obstruction set.
%
%  Now suppose $\Dn[k+2]\in \Cqk(\qFour)$ then it follows that there has to
%  exist at least one obstruction set $W \in \Deltak(\qFour,\Dn[k+2])$. We pick
%  the minimum $i$ such that there is some obstruction set in $i^{th}$ step of
%  $\Deltak(\qFour,\Dn[k+2])$ computation. Note that $i=0$ is not possible since
%  obstruction sets do not contain a solution to $\qFour$. Thus, to obtain a
%  contradiction, we will show that if there is an obstruction set in
%  $\Deltak(\qFour,\Dn[k+2])$ at $i^{th}$ step, then there has to exist an
%  obstruction set in $\Deltak(\qFour,\Dn[k+2])$ in $(i-1)^{th}$ step.
%\end{proofsketch}
For showing this, we first need to set up some definitions and prove some useful properties.
\AP
\knowledgenewrobustcmd{\allB}{\cmdkl{\mathbb{B}}}
When $\Dn$ is clear from the context, we denote $\intro*\allB \defeq \{B_1,\ldots B_n\}$ and, for every $1\le j \le n-1$, we denote
\knowledgenewrobustcmd{\allE}[1]{\cmdkl{\mathbb{E}^{#1}}}
\AP
$\intro*\allE{j} \defeq \{ E^j_l \mid 1\le l \le n-3\}$ 
where the $B_i$'s and $E^j_l$'s are the "blocks" of $\Dn$ defined above.

\AP
If $\XX =\{X_1, \dotsc, X_k\}$ is a set of "blocks" of $\Dn$, a set of "facts" $W = \{ w_1,\ldots w_k\}$ is called a ""partial repair"" of $\XX$
if $w_i\in X_i$ for every $1\le i \le k$. 
\knowledgenewrobustcmd{\Wprep}[1]{\cmdkl{W[}#1\cmdkl{]}}
\AP We denote by $\intro*\Wprep{\allE{j}}$ to be the set
of "facts" from $W$ in the "blocks" $\XX \cap \allE{j}$ (for $1\le j\le n-1$),
and $\reintro*\Wprep{\allB}$ to be the set of facts from $W$ in the "blocks" $\XX \cap \allB$.





Recall that for every $3\le l \le n-2$ and every $1\le j\le n-1$ we have $b^j_l \in B_l$
and the "triangle" $\{b^j_l, u^j_{l-1}, v^j_{l-2}\}$.
%formed by $\set{a^j_l, e^j_{l-1}, e^j_{l-2}}$. 
For each such $j$ and $l$ we define 
\knowledgenewrobustcmd{\back}{\cmdkl{U}}
\knowledgenewrobustcmd{\front}{\cmdkl{V}}
\AP
$\intro*\back(j,l) \defeq \{ u^j_k \mid 1\le k \le l-2\}$ and
$\intro*\front(j,l) \defeq \{ v^j_k \mid l-1 \le k \le n-3\}$, which are depicted in \Cref{fig:counterexample:U-V}. 

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{img/counterexample-U-V.pdf}
  \caption{Depiction of $\back(j,l)$ as  green solid discs, and $\front(j,l)$ as  blue solid discs.}
  \label{fig:counterexample:U-V}
\end{figure}




Intuitively, $\back(j,l)$ and $\front(j,l)$ represent the "facts" that need to be picked in "blocks" of $\allE{j}$ if one wants to construct a "repair" of $\Dn$ containing $b_l^j$ and having no query "solutions".
In "fact" note that $\back(j,l) \cup \front(j,l)$ picks exactly one "fact" for every "block"
in $\allE{j}$. But $u^j_{l-1},~v^j_{l-2} \not\in \back(j,l) \cup
\front(j,l)$. Consequently, there are no "solutions" in the set of "facts"
$\back(j,l)\cup \front(j,l)\cup \{ b^j_l\}$.

Similarly, recall that for every $1\le j\le n-1$, $\Dn$ contains the "triangle" $\{b^j_1, b^j_2, u^j_1\}$, so if a "repair" contains 
either $b^j_1$ of $b^j_2$ and contains no "solution" to $\qFour$, this "repair" must pick no $u$ "fact" in the "blocks" of $\allE{j}$. Thus, we define
 $\back(j,1) = \back(j,2) = \emptyset$ and
$\front(j,1) = \front(j,2) = \{ v^j_k \mid 1 \le k \le n-3\}$, so that there are no "solutions" in the set of "facts"
$\back(j,l)\cup \front(j,l)\cup \{ b^j_l\}$, for $l\in\{1,2\}$.

Dually,
$\{b^j_{n-1}, b^j_{n}, v^j_{n-3}\}$ form a "triangle", so define
$\back(j,n) = \back(j,n-1) = \{ u^j_k \mid 1\le k \le n-3\}$ and
$\front(j,n) = \front(j,n-1) = \emptyset$. Again
there are no "solutions" in the set of "facts"
$\back(j,l)\cup \front(j,l)\cup \{ b^j_l\}$, for $l\in\{n-1,n\}$.

%\red{The intuition for defining $\back(j,l)$ and $\front(j,l)$ are as
%  follows. Consider some $1\le j \le n-1$ and $3\le l \le n-3$. Then the fact
%  $b^j_l$ forms a triangle with $v^j_{l-2} ,~u^j_{l-1}$. Since every "block" of
%  the form $E^j_k$ is of size $2$, it can be verified that
%  $\{ b^j_l,~ u^j_k\} \in \Deltak[2](q,\Dn)$ for every $1 \le k\le l-2$. So, for
%  a given $j,l$ we collect the set of all $u^j_k$ for $1 \le k\le l-2$ in
%  $\back(j,l)$. Similarly, it can be verified that
%  $\{b^j_l, v^j_k\} \in \Deltak[2](q,\Dn)$ for every $l-1 \ge k \le n-3$. Hence,
%  we collect the set of all $v^j_k$ where $l-1 \le k \le n-3$ in
%  $\front(j,l)$. Finally, $\back(j,1),\back(j,2), \front(j,1), \front(j,2)$ and
%  $\back(j,n),\back(j,n-1),\front(j,n), \back(j,n-1)$ handle the corner cases.}
%  \sidediego{I'm not sure what the color red means here, but I didn't understand at all the red intuition. I think we can remove it...}
%
 Overall, for every $1\le l \le n$ and every $1\le j\le n-1$ we have:
 \begin{align*}
  \begin{aligned}
    &\text{$\back(j,l)\cup \front(j,l)\cup \{ b^j_l\}$ forms a "partial repair" over the
    "blocks" $\{B_l\} \cup \allE{j}$, and } \\
    &\text{$\back(j,l)\cup \front(j,l)\cup \{ b^j_l\}$ contains no "solution".} 
    \end{aligned}
 \end{align*}
%\sidediego{\eqref{hyp:partial} labeled but never used...}
 
 
% \bigskip
% \sidediegoh{Given a set of "blocks" $X = \{ X_1,\ldots X_k\}$ of $\Dn$, we denote $X[\allB]$
% to be the set of all "blocks" in $X\cap \allB$.  Similarly, for every
% $1\le j \le k-1$ we denote $X[\allE{j]}$ to be the set of all "blocks" that occur
% in $X \cap \allE{j}$.}{Is this a wordy way of saying $X[\allB] = X \cap \allB$ and $X[\allE{j]} = X \cap \allE{j}$? Do we gain something with this extra notation?}
 
\AP
A set of "facts" $W$ of size $k$ is called a ""$k$-obstruction set"" if $W$ is
a "partial repair" of some $\XX = \{X_1,\ldots X_k\}$ and if
$\XX \cap \allB = \{B_{i_1},B_{i_2}\ldots B_{i_l}\}$ for some $l\le k$ with
$\Wprep{\allB} = \{ b^{j_1}_{i_1}, b^{j_2}_{i_2}\ldots b^{j_l}_{i_l}\}$, then the
following conditions hold:
\begin{enumerate}
\item \label{condneq}  $j_1,j_2,\ldots j_l$ are pairwise distinct. 

\item \label{condt} For every $1\le m \le l$ we have
  $\Wprep{\allE{j_m}} \subseteq \back(j_m,i_m) \cup \front(j_m,i_m)$.


\item \label{condj} For every $1\le j \le n-1$ there exists $1\le l \le n$ such that
  $\Wprep{\allE{j}} \subseteq \back(j,l) \cup \front(j,l)$.
\end{enumerate}

\begin{lem}
\label{lemma-no solution in obstruction}
If $W$ is a "$k$-obstruction set", then there are no "solutions" to the query $\qFour$
within $W$.
\end{lem}
\begin{proof}
  Let $W$ be a "partial repair" of $\XX = \{X_1,\ldots X_k\}$. By
  condition~\eqref{condj}, for every $1\le j \le n-1$ there are no "solutions"
  within $\Wprep{\allE{j}}$. By construction, it is also not possible to have
  "solutions" involving one "fact" from $\Wprep{\allE{j}}$ and another from
  $\Wprep{\allE{j'}}$ for $j\ne j'$ (\cf~Figure~\ref{fig:counterexample}).

  So if a "solution" exists, it has to involve some "fact" of the form
  $b^j_l \in \Wprep{\allB}$. By construction of $\Dn$ this "solution" must involve  either
  $u^j_{l-1}$ or $v^j_{l-2}$. But by 
  Condition~\eqref{condt} none of them are in $W$.
\end{proof}


\vspace{1cm}

We are now in shape to prove \Cref{prop-Dk not in Delta(k-2)}.
\begin{proof}[Proof of \Cref{prop-Dk not in Delta(k-2)}]
  It will be a consequence of the following two claims:
  %
  \begin{clm}
    \label{claim1} For every set of $k$ "blocks" $\XX = \{X_1,\ldots X_k\}$ of $\Dn[k+2]$, there exists  a "partial repair" $W$ of $\XX$ such that $W$ is a "$k$-obstruction set".
  \end{clm}
  %
  \begin{clm}
    \label{claim2} For every set of "facts" $W$, if $W$ is a "$k$-obstruction set", then $W\not\in \Deltakp(\qFour,\Dn[k+2])$.
  \end{clm}
  %
  The two claims together imply that for every set of "blocks"
  $\set{X_1, \dotsc, X_k}$ of $\Dn[k+2]$ there exists a "partial repair" $W$ for
  $\set{X_1, \dotsc, X_k}$ such that $W\not\in \Deltakp(\qFour,\Dn[k+2])$. Hence,
  $\Dn[k+2]\not\models \Cqkp(\qFour)$. Hence, we are only left with the proofs of Claims \Cref{claim1,claim2}.
\end{proof}


\begin{proof}[Proof of \Cref{claim1}] Recall that $\Dn[k+2]$ has $k+2$ "blocks"
of the form $B_i$ and each $B_i$ has $k+1$ "facts". Further, for every
$1 \le j \le k+1$ we have the sets of "blocks" of the from
$E^j_1\ldots E^j_{k-1}$.

First let $\XX \cap \allB = \{ B_{i_1},\ldots B_{i_m}\}$ for some $m \le k$ and
$i_1,i_2\ldots i_m \le k+2$. We let $W$ to contain
$\set{b^1_{i_1},b^2_{i_2},\ldots b^m_{i_m}}$. Moreover for every $1\le j \le m$
we add to $W$ the "partial repair" induced by $\back(j,i_j) \cup \front(j,i_j)$. That is, we add $(\back(j,i_j) \cup \front(j,i_j)) \cap {\bigcup} \XX$ to $W$ ("ie", all "facts" of $\back(j,i_j) \cup \front(j,i_j)$ that are in a "block" of $\XX$). This ensures that conditions~\eqref{condneq} and~\eqref{condt} are satisfied.

Now for all $m < j \le k+1$ we add to $W$ the "partial repair" induced by
$\front(j,1)$ ("ie", $\front(j,1) \cap {\bigcup} \XX$).  Hence, condition~\eqref{condj} is also satisfied and $W$ is a "$k$-obstruction set".
\end{proof}

\begin{proof}[Proof of \Cref{claim2}] Let $\reintro*\Deltakp(\qFour,\Dn[k+2],i)$ be
  the set computed by the algorithm of $\Cqkp(\qFour)$ at step~$i$ of the fixpoint computation.


  Suppose the claim is false, and let $n$ be the least index such that
  $W\in \Deltakp(\qFour,\Dn[k+2],n)$ for some "$k$-obstruction set" $W$ over the
  "blocks" $\XX=\set{X_1,\ldots, X_k}$.
% Let $X=\set{X_1,\ldots, X_k}$ be the "blocks" containing a fact in $W$.

  Note that $n=0$ is not possible since $W$ does not contain any "solution"
  (refer \Cref{lemma-no solution in obstruction}); hence $n >0$. By definition
  of $\Deltakp(\qFour,\Dn[k+2],n)$, this implies that there exists a set of "facts" $A$ such that
  $A$ is a "block" in $\Dn[k+2]$ or
  $A = \set{ b \in D : D \models q(ab) \lor q(ba) \lor a=b }$ for some fact
  $a\in \Dn[k+2]$ where $A\not\in \XX$ (if $A$ is a "block") and for all
  $a\in A$ there is a subset $W'\subseteq W\cup\{a\}$ of size at most $k$ such
  that $W'\in \Deltakp(\qFour,\Dn[k+2],n-1)$ and further $W'$ is not a
  "$k$-obstruction set", nor a subset thereof.

  Let $\XX \cap \allB = \{B_{i_1},\ldots B_{i_m}\}$ for some $m\le k$ and
  $\Wprep{\allB} = \{b^{j_1}_{i_1},b^{j_2}_{i_2},\ldots b^{j_m}_{i_m}\}$. So there
  exists $k+1-m$ many distinct indices $j$ that are not in
  $\set{j_1, \dotsc, j_m}$.  Let $j_{m+1}, \dotsc, j_{k}, j_{k+1}$ be those
  indices. Since $\XX$ is of size $k$, among those indices there can be at most
  $k-m$ many indices $s$ such that $\XX \cap \allE{s} \ne \emptyset$. Thus,
  there exists at least one index $s$ such that $s\not\in \set{j_1,\ldots j_m}$
  and $\XX \cap \allE{s} = \emptyset$.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{img/counterexample-3cases.pdf}
  \caption{"Database" $\Dn[k+2]$ in the proof of Claim~\ref{claim2}, with  "$k$-obstruction set" $W$ over "blocks" $\XX$. Dotted-line boxes depict the "block" $A$ in cases a) b) and c) of the proof.}
  \label{fig:counterexample:3cases}
\end{figure}
Now we consider various candidates for $A$ and show that each case leads to a contradiction.
 %
\begin{itemize}
\item If $A = B_l$ for some $1\le l\le k+2$ then consider $b_l^{s} \in
  B_l$. Observe that every "$k$-set" over $W \cup \{ b_l^{s}\}$ forms a
  "$k$-obstruction set" since condition~\eqref{condt} holds vacuously for
  $s$. Hence, there must exist a "$k$-obstruction set" inside
  $\Deltakp(\qFour,\Dn[k+2],n-1)$, which is in contradiction with the
  minimality of $n$.

\item If, otherwise, $A=E^\lambda_l$ for some $1\le \lambda \le k+1$ and $1\le
  l \le k-1$, there are three cases to consider depending on where $A$ lies in relation to $\XX$ (see Figure~\ref{fig:counterexample:3cases}):
\begin{itemize}
\item[a)] If $\lambda \in \set{j_1,\ldots j_m}$, say $\lambda = j_t$, then by condition~\eqref{condt}
  $\Wprep{\allE{\lambda}} \subseteq \back(j_t,i_t) \cup \front(j_t,i_t)$. Let $w$ be the
  "fact" in $E^\lambda_l$ picked by $\back(j_t,i_t) \cup \front(j_t,i_t)$. Then every
  $k$-sized subset of $W\cup \{ w\}$ is a "$k$-obstruction set" (all conditions
  follow since $W$ is already a "$k$-obstruction set"). This is in contradiction with the minimality of $n$.

\item[b)] If $\lambda \not\in \set{j_1,\ldots j_m}$ but $\XX \cap \allE{r} \ne \emptyset$ then by
  condition~\eqref{condj}, $\Wprep{\allE{\lambda}} \subseteq \back(\lambda,\lambda')\cup \front(\lambda,\lambda')$ for some
  $1\le \lambda'\le k+2$. Let $w$ be the "fact" in $E^\lambda_l$ picked by
  $\back(\lambda,\lambda')\cup \front(\lambda,\lambda')$. Then, again every $k$-size subset of
  $W\cup \{ w\}$ is a "$k$-obstruction set" (all conditions follow since $W$ is
  already a "$k$-obstruction set"). This is a contradiction.

\item[c)] Otherwise, $\lambda\not\in \set{j_1,\ldots j_m}$ and $\XX \cap \allE{\lambda} = \emptyset$. In this
  case, pick $v^\lambda_l\in E^\lambda_l$ for some arbitrary $l$. We have
  $\{v^\lambda_l\} \subseteq \back(\lambda,1) \cup \front(\lambda,1)$. Hence, it can be verified
  that every $k$-sized subset of $W \cup \{v^\lambda_l\}$ is a "$k$-obstruction set",
  which again is a contradiction.
\end{itemize}
\item Otherwise $A =  \set{ b \in D : D \models q(ab) \lor q(ba) \lor a=b }$ for some fact $a\in \Dn[k+2]$ which implies that $A=\set{b^\lambda_l, u^\lambda_{l-1}, v^\lambda_{l-2}}$. The argument is similar to the previous case.
  \begin{itemize}
\item[a)] If $\lambda\in \set{j_1,\ldots j_m}$, say $\lambda = j_t$, then by condition~\eqref{condt}
  $\Wprep{\allE{\lambda}} \subseteq \back(j_t,i_t) \cup \front(j_t,i_t)$. Let $w$ be the
  "fact" in $A$ picked by $\back(j_t,i_t) \cup \front(j_t,i_t)$. Then every
  $k$-sized subset of $W\cup \{ w\}$ is a "$k$-obstruction set" (all conditions
  follow since $W$ is already a "$k$-obstruction set"). This is in contradiction with the minimality of $n$.

\item[b)] If $\lambda\not\in \set{j_1,\ldots j_m}$ but $\XX \cap \allE{r} \ne \emptyset$ then by
  condition~\eqref{condj}, $\Wprep{\allE{\lambda}} \subseteq \back(\lambda,\lambda')\cup \front(\lambda,\lambda')$ for some
  $1\le \lambda'\le k+2$. Let $w$ be the "fact" in $A$ picked by
  $\back(\lambda,\lambda')\cup \front(\lambda,\lambda')$. Then, again every $k$-size subset of
  $W\cup \{ w\}$ is a "$k$-obstruction set" (all conditions follow since $W$ is
  already a "$k$-obstruction set"). This is a contradiction.

\item[c)] Otherwise, $\lambda\not\in \set{j_1,\ldots j_m}$ and $\XX \cap \allE{\lambda} = \emptyset$. In this
  case, pick $v^\lambda_{l-2}\in A$. We have
  $\{v^\lambda_{l-2}\} \subseteq \back(\lambda,1) \cup \front(\lambda,1)$. Hence, it can be verified
  that every $k$-sized subset of $W \cup \{v^\lambda_l\}$ is a "$k$-obstruction set",
  which again is a contradiction.\qedhere
\end{itemize}
\end{itemize}
\end{proof}
%From Proposition~\ref{prop-Dk not in Delta(k-2)} and Lemma~\ref{lem:cert-triangle-ptime} we immediately get the following:



As we have seen, $\certain(\qFour)$ cannot be computed using our fixpoint
algorithm. 
\AP
We will next show that $\certain(\qFour)$ is in polynomial time, by
reduction to the ""Saturating Bipartite Matching problem"" (or ""SBM problem"" for short). This is the problem of, given bipartite graph $(V_1 \cup V_2, E)$, whether there is an injective function $f: V_1 \to V_2$ such that $(v,f(v)) \in E$ for every $v \in V_1$. The "SBM problem" is known to be in \ptime~\cite{DBLP:journals/siamcomp/HopcroftK73}, although its precise complexity class is unknown to this day.



\begin{thm}\label{lem:cert-triangle-ptime}
  $\certain(\qFour)$ is in \ptime.
  Moreover, there is a \logspace-reduction from $\certain(\qFour)$ to the "SBM problem".
\end{thm}
\begin{proof}
Fix an input "database" $D$. We reduce $\certain(\qFour,D)$ to the "SBM problem".
 
First we check for self-loops in $D$. If there is a "fact" $a \in D$ such that
$D\models q(aa)$ then we first check if $a$ is a singleton "block". If so, then
$D \models \certain(\qFour)$. Otherwise, $D \models \certain(\qFour)$ iff
$D\setminus\set{a} \models \certain(\qFour)$, so we can consider a smaller
"database" and repeat the argument.  So assume that there is no "fact"
$a \in D$ such that $ D\models \qFour(aa)$.
    
% Since $\qFour$ contains only two
% atoms, for a "database" $D$, it is convenient to describe the set of solutions to
% $\qFour$ as a graph. More precisely we say that the "facts" $a,b \in D$ are
% \emph{$\qFour$-related} if $D\models \qFour(ab)$ or $D\models \qFour(ba)$.  
% From the properties of $\qFour$ it follows that every connected component in $\solgraph$ is
% always a clique of size less than or equal to $3$.

Now consider the bipartite graph $G = (V_1 \cup V_2, E)$ where $V_1$ is the set
of all "blocks" of $D$ and $V_2$ is the set of all maximal cliques in the "solution graph" 
$\solgraph$. Note that, by property \eqref{shape-solgraph-q4} (in page
\pageref{shape-solgraph-q4}), $V_2$ forms a partition of $D$, namely the set of
all maximal connected components of $\solgraph$. Let $(v_1,v_2) \in E$ if the
"block" $v_1$ contains a "fact" which is in the clique $v_2$.

  
\AP
Suppose that there is a ""$V_1$-saturating matching"", that is, an injective
 function $f: V_1 \to V_2$ such that $(v_1,f(v_1)) \in E$ for every
 $v_1 \in V_1$. We construct a "repair" $r$ where for every "block" $B$ of $D$, we
 pick the "fact" (or one of the "facts", if there are more than one) which is in
 $f(B)$. In this way, no two chosen "facts" will be in the same clique, and also
 since there is no "solution" of the form $\qFour(aa)$ in $D$, no two chosen "facts"
 will form a "solution" to $\qFour$. Thus, $r\not\models \qFour$.

Conversely, if $\qFour$ is not "certain" in $D$, let $r$ be a "repair" such that $r \not\models \qFour$. For each "block" $B$ of $D$ let $r(B)$ be the "fact" of $B$ belonging to $r$.
Note that, since $V_2$ is a partition of $D$, each $r(B)$ belongs to a unique clique in $V_2$.
Define $f: V_1\to V_2$ such that each "block" $B \in V_1$ is mapped to the clique in $V_2$ where $r(B)$ lies. To verify that $f$ is a witness function of a 
"$V_1$-saturating matching" for $G$, note that for every $B \in V_1$ we have $(B, f(B)) \in E$, as $B$ and $f(B)$ both contain $r(B)$. Moreover, $f$ is injective, otherwise if $f$ maps two distinct "blocks" to the same clique, this clique must contain at least two "facts" $a,b$ from $r$. These two "facts" are neighbors in $\solgraph$, and then $r \models \qFour(ab)$ or $r \models \qFour(ba)$, contradicting the hypothesis $r \not\models \qFour$.

Thus, to check if $D\in \certain(\qFour)$, it is sufficient to check if there is a "$V_1$-saturating matching" for $G$.
\end{proof}


As we show next, $\certain(\qFour)$ turns out to be \emph{equivalent} to the
complexity of the "SBM problem" under \logspace-reductions. The complexity for
the "SBM problem" is a long-standing open problem, and hence the precise
complexity of $\certain(\qFour)$ remains open.

\begin{thm}
  $\certain(\qFour)$ is complete for the "SBM problem" under \logspace-reductions.
  \end{thm}
  \begin{proof}
    \Cref{lem:cert-triangle-ptime} shows the reduction to the "SBM problem". We now prove the other direction. 
  
  Given a bipartite graph $G = (V_1\cup V_2, E)$, let $V_1 = \{ s_1,\ldots s_n\}$ and $V_2 = \{ t_1,\ldots t_m\}$. 
  We will define a "database" $D_G$ such that there exists a "$V_1$-saturating matching" in $G$ if{f} $\qFour$ is not "certain" in $D_G$. 
    
  \knowledgenewrobustcmd{\Neighbour}{\cmdkl{N}}
  \AP
  For all $s_j\in V_1$ let $\intro*\Neighbour(s_j) \subseteq V_2$ denote the neighbours of $s_j$ and similarly for all $t_i \in V_2$ let $\reintro*\Neighbour(t_i)\subseteq V_1$ denote the neighbours of $t_j$.
  
  First note that if there is some $s_j\in V_1$ such that $\Neighbour(s_j) = \emptyset$, then clearly there cannot be a "$V_1$-saturating matching". So assume that for every $s_j\in V_1$, $\Neighbour(s_j) \ne \emptyset$. Similarly, if there is some $t_i\in V_2$ such that $\Neighbour(t_i) = \emptyset$, then $t_i$ does not contribute to any matching and hence can be removed from the input. So we can also assume that for every $t_i\in V_2$, $\Neighbour(t_i) \ne \emptyset$.
  Further,  suppose there is some $t_i$ such that $|\Neighbour(t_i)| = 1$, let $s_j$ be the single neighbour of $t_i$. In this case, if there exists a "$V_1$-saturating matching", then there is one such matching where $s_j$ is mapped to $t_i$. So we can remove the pair $(s_j,t_i)$ from the input graph. This means that we can assume that for every $t_i\in V_2$, $|\Neighbour(t_i)| \ge 2$.
  
  
  Altogether, we have $|\Neighbour(s_j)| \ge 1$ for all $s_j\in V_1$ and $|\Neighbour(t_i)| \ge 2$ for all $t_i\in V_2$. Note that these  properties can be checked in \logspace. 
  
  
  Now we define the  "database" $D_G$. Note that this construction is very similar to the construction of $\Dn$ that we used to prove Theorem \ref{thm-X+lowerBound}.
  \begin{itemize}
  \item For every vertex in $s_j\in V_1$ create a "block" $B_j$ in $D_G$.
  \item For every $s_j\in V_1$ and $t_i\in V_2$, if $t_i\in \Neighbour(s_j)$ then there is a "fact" denoted by $b^i_j$ in the "block" $B_j$. By assumption $\Neighbour(s_j) \ge 1$ and hence every "block" $B_j$ is non-empty.
  \item For every $t_i\in V_2$ if $|\Neighbour(t_i)| = l$ then let $s_{i_1},\ldots s_{i_l} \in V_1$ be the neighbours of $t$. By the above construction, for every $j\le l$,  there is a "fact" of the form $b^i_{i_j}$ in $B_{i_j}$ that corresponds to the vertex $t_i$.
  
  Now if $l=2$ then define $b^i_{i_1}$ and $b^i_{i_2}$ such that they form a "solution" to $\qFour$. Otherwise, if $l = 3$ then define $b^i_{i_1}, b^i_{i_2}$ and $b^i_{i_3}$ such that they pair-wise form a "solution" to $\qFour$ (the three facts form a "triangle").
  
  If $l\ge 4$ then create $l-3$ new "blocks" denoted by $E^i_1,\ldots E^i_{l-3}$ where each $E^i_j$ contains exactly two "facts" $u^i_j$ and $v^i_j$. Moreover, in the same way as described in the definition of $\Dn$ earlier (\cf~\Cref{fig:counterexample:triangles,fig:counterexample}), define the "facts" appropriately such that $\{b^i_{i_1},b^i_{i_2},u^i_1\}$ and $\{b^i_{i_{l-1}},b^i_{i_l},v^i_{l-3} \}$ form "triangles" and for every $1\le j< l-3$ we have a "triangle" $\{v^i_j,u^i_{j+1},b^i_{j+2}\}$.
  
  \end{itemize}
  The reader can verify that this is exactly the construction used to define $\Dn$. 
  \AP
  Again, this construction is in \logspace. For each such $j$ and $l$  define 
  $\intro*\back(i,l) \defeq \{ u^i_k \mid 1\le k \le l-2\}$ and
  $\intro*\front(i,l) \defeq \{ v^i_k \mid l-1 \le k \le l-3\}$,
  
  Now suppose there is a "$V_1$-saturating matching" then let us show that $\qFour$ is not "certain" for $D_G$. Consider the "repair" $r$  where for each "block" $B_j$ we  pick $b^i_j$ if $s_j$ is matched with $t_i$. Further, pick $\back(i,l) \cup \front(i,l)$ which gives a "partial repair" over $E^i_1\ldots E^i_l$.
  
  If some $t_i \in V_2$ is not matched with any vertex in $V_1$ then pick $\back(i,1) \cup \front(i,1)$ which gives a "partial repair" over $E^i_1\ldots E^i_l$.  It can be verified that the obtained "repair" does not contain any "solution".
  
  Finally, suppose there is a "repair" $r$ of $D_G$ that falsifies $\qFour$, and let us show that there is a "$V_1$-saturating matching" in $G$.
  For any such "repair" $r$, note that if $b^i_j$ is picked in "block" $B_j$ then for all other "blocks" $B_{j'}$, the "fact" $b^i_{j'}$ cannot be in $r$ since that would make $\qFour$ true. Also $b^i_j\in B_j$ only if there is an edge between $s_j$ and $t_i$. Hence, we can define the "$V_1$-saturating matching" that maps every $s_j\in V_1$ to $t_i\in V_2$, where  $b^i_j$ is the "fact" in $r$ from the "block" $B_j$.
  \end{proof}



\subsubsection{The case of $\qFive$}

We now show that $\certain(\qFive)$ cannot be computed by $\Cqk(\qFive)$. This
is shown by reduction to the case of $\qFour$ based on the following construction:

\begin{prop}
\label{theorem-UnconditionX+-Lowerbound-sjf}
For every "database"  $D$ over the "signature" of $\qFour$ we can construct a
"database" $D'$ over the "signature" of $\qFive$ such that:
\begin{enumerate}
\itemAP if $D\models \certain(\qFour)$  then $D'\models \certain(\qFive)$ \label{theorem-UnconditionX+-Lowerbound-sjf:1}
\itemAP For every $k\ge 2$, if $D'\models \Cqk(\qFive)$ then
  $D\models \Cqkp(\qFour)$. \label{theorem-UnconditionX+-Lowerbound-sjf:2}
\end{enumerate}
\end{prop}

\begin{proof}
  Let $D$ be a "database" over the "signature" of $\qFour$.

 \luc{Careful! The reduction has to preserve X+, so we cannot assume that the
   database is self-loop free or any other fancy things. That would be OK for a
 logspace reduction but not for what we need. So I revisited entirely the proof
for taking care of the degenerated cases, please verify.}

  
  Consider the "solution graph" $\solgraph$ of $D$. Recall that by property
  \eqref{shape-solgraph-q4}, every connected component in $\solgraph$ is always
  a clique of size at most $3$. Thus, every "fact" of $D$ can be part of
  exactly one maximal clique.

  Let $B_1,B_2\ldots B_m$ be the set of all "blocks" of $D$ and
  $C_1,C_2\ldots C_l$ be the set of cliques in $\solgraph$. Let
  $e_1,e_2\ldots e_m, f_1,f_2\ldots f_l$ be fresh and pairwise distinct domain
  elements.  Define $D'$ as follows:
\begin{itemize}
\item \label{item-uncond-preserves-certain} For every "fact"
  $u$ occurring in a block $B_i$ of $D$ and in the clique $C_n$ add the "fact"
  $u_{R_1}= R_1(\underline{e_i}\, f_n)$ to $D'$. Notice that there could be two
  distinct facts occurring in the same block of $D$ and in the same
  clique. They are then both associated to the same fact of $D'$.
  
\item
  \label{item-uncond-preserves-X+} For every two facts $u,v$ from a
  clique $C_n$ such that $D\models \qFour(uv)$ and $u,v$ are in two distinct
  "blocks" $B_i$ and $B_j$, create two new "facts" in $D'$ as
  $u^v_{S_1}=S_1(\underline{f_ng}~e_i)$ and
  $v^u_{S_1}=S_1(\underline{f_ng}~e_j)$, where $g$  is a fresh element depending only on $u$ and $v$.
\item
  \label{item-uncond-preserves-X+-2} For every facts $u$ from a
  clique $C_n$ and a block $B_i$ such that $D\models \qFour(uu)$ create a new "facts" in $D'$ as
  $u^u_{S_1}=S_1(\underline{f_ng}~e_i)$, where $g$  is a fresh element depending only on $u$.
\end{itemize}

\luc{We need a picture for illustrating the construction}

Notice that for any two "facts" $u,v \in D$ if
$D\models \qFour(uv)$ and $u,v$ are in two distinct blocks, then $u^v_{S_1}\simblock v^u_{S_1}$,
$D'\models \qFive(u_{R_1}u^v_{S_1}) \land \qFive(v_{R_1}v^u_{S_1})$, and the
"block" containing $u^v_{S_1},v^u_{S_1}$ in $D'$ does not contain any other
fact.
Moreover if for some fact  $u \in D$, $D\models \qFour(uu)$ then $D'\models
\qFive(u_{R_1}u^u_{S_1})$  and the
"block" containing $u^u_{S_1}$ in $D'$ does not contain any other
fact.
Finally, the only solutions in $D'$ for $\qFive$ are of the form
$\qFive(u_{R_1}u^v_{S_1})$ for some "facts" $u,v\in D$ such that
$D\models \qFour(uv)$ and $u \not\simblock v$ or $u=v$. Now we prove both claims of
the statement.

\medskip

\proofcase{\eqref{theorem-UnconditionX+-Lowerbound-sjf:1}} Suppose
$D\models \certain(\qFour)$. To verify that $D'\models \certain(\qFive)$, pick
any "repair" $r'$ of $D'$. By construction, every $R_1$-"fact" $a$ of $r'$ is of the form $u_{R_1}$
for some "fact" $u$ in $D$. Recall that there could be two such facts $u$. We
arbitrarily select one of them that we denote by $f_R(a)$.

Consider the set $r = \set{u \mid \exists a \in r' ~ u=f_R(a)}$. First, we claim that $r$
is a "repair" of $D$. To see this, suppose $r$ contains two facts $u,v\in r$
such that $u\simblock v$ then both $u,v$. By construction of $r$, $u=f_R(a)$
and $v=f_R(b)$ for some facts $a,b$ of $r'$. By construction of $D'$, it
follows from $u\sim v$ that $a\sim b$ and therefore $a=b$ as $r$ is a
repair. Hence $u=v$. further for every
"block" $B_i$ in $D$ there is a $R_1$-"block" in $D'$ whose facts have key
$e_i$ and one of those facts is picked in $r'$. Thus $r$ is a "repair" of
$D$. By assumption, there is some $u,v\in r$ such that $D\models \qFour(uv)$.

If $u=v$ by construction of $r$, $u_{R_1} \in r'$. As $u^u_{S_1}$ is in any
repair of $D'$, $r'\models \qFive(u_{R_1} u^u_{S_1})$ as desired.

If $u\neq v$, by construction of $r$, $u_{R_1},v_{R_1}\in r'$, and $\set{u^v_{S_1}, v^u_{S_1}}$ form a
$S_1$-"block" in $D'$. Hence, $r'$ contains one of
$\set{u^v_{S_1}, v^u_{S_1}}$. If $u^v_{S_1}\in r'$ then
$r'\models \qFive(u_{R_1}u^v_{S_1})$; otherwise if $v^u_{S_1}\in r'$ then
$r'\models \qFive(v_{R_1}v^u_{S_1})$.
  
  \bigskip


  \proofcase{\eqref{theorem-UnconditionX+-Lowerbound-sjf:2}}
Fix some $k\ge 2$.  Let $\reintro*\Deltakp(\qFour,D,i)$ and $\reintro*\Deltak(\qFive,D',i)$ be the
  sets computed at step $i$ of $\Cqkp(\qFour)$ and $\Cqk(\qFive)$
  respectively. First we prove the following claims.

\begin{clm}\label{claim-R-block-only}
  Let $u,v,w$ be facts of $D$ in the same clique of the "solution graph"
  $\solgraph$. Possibly $v \sim w$ or $v=w$ but we assume $u\not\sim v$ and $u\not\sim w$. In particular
  $D\models \qFour(uv) \lor \qFour(vu)$. Then for every "$k$-set" $S$ over $D'$, if
  $S\cup \set{u^v_{S_1}} \in \Deltak(\qFive,D',i)$ then
  $S \cup \set{v_{R_1}} \in \Deltak(\qFive,D',i+1)$ and
  $S \cup \set{w_{R_1}} \in \Deltak(\qFive,D',i+1)$.
\end{clm} 
Note that in the case where $v_{R_1}\in S$ the claim implies
$S\in \Deltak(\qFive,D',i+1)$. Similarly for $w_{R_1}$.

\begin{proof}[Proof of Claim] We do the case where $D\models \qFour(uv)$ the case where
  $D\models \qFour(vu)$ is symmetric.

  Assume $S\cup \set{u^v_{S_1}} \in \Deltak(\qFive,D',i)$. If
  $S \in \Deltak(\qFive,D',i)$ then the conclusion is clear. So we assume
  $S \not\in \Deltak(\qFive,D',i)$.
  We first prove that $S \cup \set{v_{R_1}} \in \Deltak(\qFive,D',i+1)$.
  The proof is by induction on $i$.

  When $i=0$ then $S\cup\set{u^v_{S_1}}\in \Deltak(\qFive,D',0)$ and
  $S\not\in\Deltak(\qFive,D',0)$. This can only happen  if $u_{R_1}\in S$. Let $B'$ be the "block" of
  $u^v_{S_1}$. A simple analysis shows that the "block" $B'$ is a witness for
  $S\cup\set{v_{R_1}} \in \Deltak(\qFive,D',1)$.

  For the induction step, suppose
  $S\cup\set{u^v_{S_1}} \in \Deltak(\qFive,D',i)$. Let $B'$ be the "block" of $D'$
  used as the witness. If $B'$ does not contain $v_{R_1}$ then, using the
  induction, we can check that $B'$ is a witness for
  $ S \cup \set{v_{R_1}} \in \Deltak(\qFive,D',i+1)$. Now suppose $B'$ contains
  $v_{R_1}$. By definition, this implies that $S \cup \set{v_{R_1},u^v_{S_1}}$
  contains a "$k$-set" in $\Deltak(\qFive,D',i-1)$. By induction this implies that 
  $S \cup \set{v_{R_1}}$ is in $\Deltak(\qFive,D',i)$.

  It remains to show that $S \cup \set{w_{R_1}} \in \Deltak(\qFive,D',i+1)$. As
  $u,v,w$ are in the same clique, it is enough in view of the previous case to
  show that if $S\cup\set{u^v_{S_1}}\in\Deltak(\qFive,D',i)$ then
  $S\cup\set{u^w_{S_1}}\in\Deltak(\qFive,D',i)$. We do again an induction on $i$.

   When $i=0$, we have already seen above that we must have $u_{R_1} \in S$. As
   $D'\models \qFive(u_{R_1}u^w_{S_1})$ the result follows.

   For the induction step, suppose
   $S\cup\set{u^v_{S_1}} \in \Deltak(\qFive,D',i)$. Let $B'$ be the "block" of $D'$
   used as the witness. If $B'$ does not contain $u^w_{S_1}$ then, using the
   induction, we can check that $B'$ witnesses the fact that
   $ S \cup \set{u^w_{S_1}} \in \Deltak(\qFive,D',i)$. Now suppose $B'$ contains
   $u^w_{S_1}$. By definition, this implies that $S \cup \set{u^w_{S_1},u^v_{S_1}}$
   contains a "$k$-set" in $\Deltak(\qFive,D',i-1)$. By induction we conclude the
   desired result.
  \end{proof}

  Assume now that $D' \models \Cqk(\qFive)$. We need to show that
  $D\models \Cqkp(\qFour)$.

  Let $S$ be a "$k$-set" of $D'$. Let $\tilde S$ be any "$k$-set" of
  $D$ containing one "fact" $u$ as soon as $u_{R_1} \in S$ or $v^u_{S_1} \in S$
  for some "fact" $v$. We claim that if $S\in
  \Deltak(\qFive,D',i)$ then $\tilde S\in\Deltakp(\qFour,d,i+1)$.

  The proof is by induction on $i$.

  For $i=0$, if $S\in \Deltak(\qFive,D',0)$ then it contains a solution to $\qFive$
  of the form $u_{R_1}u^v_{S_1}$ for some facts $u,v$ of $D$. By construction
  $D\models \qFour(uv)$ and $u,v\in \tilde S$. Hence
  $\tilde S\in\Deltakp(\qFour,d,0)$.

  For the induction step, assume $S\in \Deltak(\qFive,D',i)$ as witnessed by a
  "block" $B'$ of $D'$. If $B'$ is a $R_1$-"block" then the block
  $\tilde B=\set{u\mid u_{R_1}\in B'}$ witnesses the fact that
  $\tilde S\in\Deltakp(\qFour,D,i)$. If $B'$ is a $S_1$-block of the form
  $\set{u^v_{S_1},v^u_{S_1}}$. Set $w$ to the third "fact" in the clique of
  $u,v$ in the "solution graph" $\solgraph$ (set $w=v$ if the clique has size
  two). From \Cref{claim-R-block-only} we get that each of
  $S\cup\set{u_{R_1}}$, $S\cup\set{v_{R_1}}$, $S\cup\set{w_{R_1}}$ contains a
  "$k$-set" in $\Deltak(\qFive,D',i-1)$. Hence by induction each of
  $\tilde S\cup\set{u}$, $\tilde S\cup\set{v}$, $\tilde S\cup\set{w}$ contains
  a "$k$-set" in $\Deltakp(\qFour,D,i)$. Hence, by the extended rule,
  $\tilde S\in\Deltakp(\qFour,D,i+1)$.
  It remains to consider the case where $B'$ is a $S_1$-block of the form
  $\set{u^u_{S_1}}$. But then $u$ is a self loop and is contained in $\tilde
  S$. By definition we then have $\tilde S \in\Deltakp(\qFour,D,0)$.

\end{proof}

\begin{thm}\label{thm-q5-cqk}
 $\certain(\qFive)$ cannot be computed by
  $\Cqk(\qFive)$, for any choice of $k$.
\end{thm}
\begin{proof}
  By means of contradiction, assume that $\certain(\qFive)$ is equivalent to $\Cqk(\qFive)$ for some $k \geq 2$. We will now show that this implies that $\certain(\qFour)$ is equivalent to $\Cqkp(\qFour)$, contradicting \Cref{thm-X+lowerBound}. 
  
  It is enough to show that if a "database" $D$ is such that $D\models\certain(\qFour)$ then
  $D\models \Cqkp(\qFour)$. Let $D'$ be the "database" constructed from $D$
  given by \Cref{theorem-UnconditionX+-Lowerbound-sjf}. As
  $D\models\certain(\qFour)$, we get from
  \Cref{theorem-UnconditionX+-Lowerbound-sjf}-\eqref{theorem-UnconditionX+-Lowerbound-sjf:1} that
  $D'\models\certain(\qFive)$. From our hypothesis it follows that
  $D'\models\Cqk(\qFive)$. By \Cref{theorem-UnconditionX+-Lowerbound-sjf}-\eqref{theorem-UnconditionX+-Lowerbound-sjf:2} this
  implies that $D\models\Cqkp(\qFour)$ as desired.
\end{proof}

\subsubsection{The case where a "self-join-free query" $q\not\models\HP$}

We finally reduce the case of $\qFive$ to any arbitrary query falsifying $\HP$. Let $q$ be a "self-join-free query" such that
$q\not\models\HP$. We show that for all $k$, if $\certain(q)$ is equivalent to
$\Cqk(q)$ then $\certain(\qFive)$ is equivalent to $\Cqk(\qFive)$, a contradiction with \Cref{thm-q5-cqk}.
The following is the analog of \Cref{theorem-UnconditionX+-Lowerbound-sjf}.

\begin{prop}
\label{proposition-q5toq}
For every "database"  $D$ for $\qFive$ we can construct a "database" $D'$
for $q$ such that:
\begin{enumerate}
\item if $D\models \certain(\qFive)$  then $D'\models \certain(q)$
\item For every $k\ge 2$, if $D'\models \Cqk(q)$ then
  $D\models \Cqk(\qFive)$.
\end{enumerate}
\end{prop}
\begin{proof}

  The construction of $D'$ from $D$ is actually taken from~\cite{DBLP:journals/tods/KoutrisW17}.

  As $q\not\models\HP$ it follows from~\cite{DBLP:journals/tods/KoutrisW17}
  that $q$ contains "atoms" $A_1$ and $A_2$ such that the following is true.
  
  \anantha{The paper \cite{DBLP:journals/tods/KoutrisW17} does not have $\HP$, it only talks about the attack grah being acyclic. How can $\lnot\HP$  imply this, since we have not yet proved that $\HP$ is equivalent to attack graph being acyclic?}

  \begin{lem}\label{lemma-conp-reduc-KW}\cite[Proof of Theorem $6.1$]{DBLP:journals/tods/KoutrisW17} \sidediego{which theorem/lemma? \\{\bf Anantha:} added, please check}
For every "database"  $D$ for $\qFive$ there is  a "database" $D'$
for $q$ and functions $f$ and $g$ such that:
\begin{enumerate}
\item If $D\models \certain(\qFive)$,  then $D'\models \certain(q)$.
\itemAP $f$ is a bijection from the $R_1$-"facts" of $D$ to the $A_1$-"facts" of
  $D'$ such that $u\simblock v$ iff $f(u)\simblock f(v)$. \label{lemma-conp-reduc-KW:bijection}
\itemAP $g$ is a function associating to any "atom" $C$ of $q$, $C\neq A_1$, and
  any $S_1$-"fact" of $D$ a $C$-"fact" of $D'$ such that:\label{lemma-conp-reduc-KW:gbijection}
  \begin{enumerate}
    \item $g$ is a bijection from $S_1$-"facts" to $A_2$-"facts" such that $u\simblock v$ if{f} $g(A_2,u)\simblock g(A_2,v)$; 
    \item for any "atom" $C\not\in\set{A_1,A_2}$, $g(C,\cdot)$ contains only one "fact".
  \end{enumerate}
  
\itemAP If $f(u)$ and $g(A_2,v)$ are part of a "solution" to $q$ in $D'$ then
  $D\models \qFive(uv)$.\label{lemma-conp-reduc-KW:last}
\end{enumerate}
  \end{lem}

  Given a "database" $D$ for $\qFive$, let $D'$ be the "database" constructed in
  \Cref{lemma-conp-reduc-KW}. In view of \Cref{lemma-conp-reduc-KW}, it remains
  to show that if $D'\models \Cqk(q)$ then $D\models \Cqk(\qFive)$.  Let
  $S'$ be a "$k$-set" in $\Delta(q,D',i)$.  Let
  $S=\set{u\mid f(u) \in D'} \cup \set{v \mid g(A_2,v) \in D'}$.  We
  claim that $S \in \Delta(q,D,i)$.

  The proof goes by induction on $i$.

  For $i=0$, $S'$ contains necessarily a "solution" to $q$ and therefore an
  $A_1$-"fact" $u'$ and an $A_2$-"fact" $v'$. Let $u$ and $v$ be such that
  $v'=g(A_2,v)$ and $u'=f(u)$. By~\Cref{lemma-conp-reduc-KW}-\eqref{lemma-conp-reduc-KW:last} this implies that
  $D\models \qFive(uv)$ and therefore $S\in\Deltaki(\qFive,D,0)$.

  For the induction step, let $B'$ be the "block" witnessing the membership of
  $S'$ into $\Delta(q,D',i)$.
\begin{itemize}
  \item Assume first that $B'$ is a $A_1$-"block". Let $B=\set{u \mid f(u)\in B'}$. By \Cref{lemma-conp-reduc-KW}-\eqref{lemma-conp-reduc-KW:bijection}
  $B$ is a "block" of $D$. We claim that it witnesses the membership
  of $S$ in $\Delta(q,D,i)$. Consider an element $b\in B$. Let $b'=f(b)$. By
  hypothesis, $S'\cup\set{b'}$ contains a "$k$-set" $T'$ in
  $\Deltak(q,D',i-1)$. By induction $T \in \Deltak(\qFour,D,i-1)$ \sidediego{$\Deltak(\qFive,D,i-1)$?} and $T$ is a
  subset of $S \cup \set{b}$. The result follows.

  \item Assume now that $B'$ is a $A_2$-"block". We conclude
  as above using $B=\set{v \mid g(A_2,v)\in B'}$ and \Cref{lemma-conp-reduc-KW}-\eqref{lemma-conp-reduc-KW:gbijection}.

  \item Finally, if $B'$ is a $C$-"block" for for some atom $C\not\in\set{A_1,A_2}$
  then $B'$ contains only one element and therefore $S'$ was actually in
  $\Delta(q,D',i-1)$ and we can conclude by induction. \qedhere
\end{itemize}
\end{proof}


\begin{thm}\label{thm-nothp-cqk}
  Let $q$ be a "self-join-free query" such that $q\not\models\HP$. Then
  $\certain(q)$  cannot be computed by
  $\Cqk(q)$, for any choice of $k$.
\end{thm}
\begin{proof}
Identical to the proof of \Cref{thm-q5-cqk} using \Cref{proposition-q5toq}
instead of \Cref{theorem-UnconditionX+-Lowerbound-sjf}.
\end{proof}




  
%%% Local Variables: 
%%% TeX-PDF-mode: t
%%% eval: (flyspell-mode t)
%%% TeX-master: "main"
%%% End: 


